FEASTS Compared with Simulations: Abnormally Irregular and Extended HI Morphologies at a Column Density of $10^{18}\,\text{cm}^{-2}$ in TNG50 and Auriga

With new atomic-hydrogen (HI) observations of FAST Extended Atlas of Selected Targets Survey (FEASTS), we present the first statistical comparison of HI morphology between observations and cosmological simulations, focusing on low-column density ($10^{18}\,\text{cm}^{-2}$) regions of Milky Way-like central galaxies. We select a 330-galaxy sample from IllustrisTNG50 (TNG50) matched to 33 FEASTS galaxies by stellar and HI masses, and mock observe them to the FAST resolution and depth at corresponding inclinations and distances for a fair comparison. In contrast to FEASTS, abnormally irregular and extended morphology is found in more than one-third of TNG50 galaxies, especially those massive and HI poor. Stellar feedback is the property that most significantly correlates with the HI morphological deviation from observations, although these deviations mostly occur at a high stellar or black-hole mass. These results indicate that in TNG50, stellar feedback significantly influences the HI morphology at $10^{18}\,\text{cm}^{-2}$, while active galactic nucleus (AGN) feedback has not so direct a role as expected. With an additional sample from Auriga, we find that the magnetic field may help HI to be more regular in its morphology, while improving the mass resolution does not alleviate the discrepancy from observation. This study reveals the potential of constraining future simulations of galaxies by observing low-column density HI.

==> figsetnote.tex <==

\figsetstart
\figsetnum{2}
\figsettitle{The \Hi moment-0 atlas of FEASTS galaxies and their distance-matched TNG50 cubes, sorted by the \Mste of FEASTS galaxies in descending order.}

\newcommand{\myfigsetgrptitle}[1]{
  The \Hi moment-0 atlas of #1 and its ten distance-matched TNG50 cubes.
}

\newcommand{\myfigsetgrpnote}[1]{
  The \Hi moment-0 atlas of #1 (the single panel above) and its distance-matched TNG50 cubes sorted by the values of morphological parameters in descending order (ten panels below).
  All panels have a sidelength of \qty{250}{\kpc}, and the beam size of \ang{;3.24;} is indicated by the circle at the lower left corner.
  On the left of #1 moment-0 map, we list its morphological parameters;
  on the right, we list the stellar and \Hi masses and the inclination.
  In the TNG panels, we list their subhalo ID, AGN-feedback mode (``K'' for kinetic mode and ``T'' for thermal mode), and morphological parameters.
  Morphological parameters listed in the atlas are not corrected for the distance.
  Contours are plotted at $\NHi=\text{\qtylist{1e18;1e19;1e20}{\per\cm\squared}}$ (solid lines) and \qty{1e21}{\per\cm\squared} (dotted lines).
}

\figsetgrpstart
\figsetgrpnum{2.1}
\figsetgrptitle{\myfigsetgrptitle{NGC~7331}}
\figsetplot{f2_1.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~7331}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.2}
\figsetgrptitle{\myfigsetgrptitle{NGC~2841}}
\figsetplot{f2_2.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~2841}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.3}
\figsetgrptitle{\myfigsetgrptitle{NGC~4565}}
\figsetplot{f2_3.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4565}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.4}
\figsetgrptitle{\myfigsetgrptitle{NGC~5907}}
\figsetplot{f2_4.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~5907}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.5}
\figsetgrptitle{\myfigsetgrptitle{NGC~3521}}
\figsetplot{f2_5.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3521}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.6}
\figsetgrptitle{\myfigsetgrptitle{NGC~4725}}
\figsetplot{f2_6.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4725}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.7}
\figsetgrptitle{\myfigsetgrptitle{NGC~6384}}
\figsetplot{f2_7.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~6384}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.8}
\figsetgrptitle{\myfigsetgrptitle{NGC~5194}}
\figsetplot{f2_8.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~5194}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.9}
\figsetgrptitle{\myfigsetgrptitle{NGC~5055}}
\figsetplot{f2_9.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~5055}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.10}
\figsetgrptitle{\myfigsetgrptitle{NGC~891}}
\figsetplot{f2_10.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~891}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.11}
\figsetgrptitle{\myfigsetgrptitle{NGC~4303}}
\figsetplot{f2_11.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4303}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.12}
\figsetgrptitle{\myfigsetgrptitle{NGC~4258}}
\figsetplot{f2_12.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4258}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.13}
\figsetgrptitle{\myfigsetgrptitle{NGC~4527}}
\figsetplot{f2_13.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4527}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.14}
\figsetgrptitle{\myfigsetgrptitle{NGC~4414}}
\figsetplot{f2_14.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4414}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.15}
\figsetgrptitle{\myfigsetgrptitle{NGC~3718}}
\figsetplot{f2_15.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3718}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.16}
\figsetgrptitle{\myfigsetgrptitle{NGC~5775}}
\figsetplot{f2_16.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~5775}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.17}
\figsetgrptitle{\myfigsetgrptitle{NGC~2903}}
\figsetplot{f2_17.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~2903}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.18}
\figsetgrptitle{\myfigsetgrptitle{NGC~5457}}
\figsetplot{f2_18.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~5457}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.19}
\figsetgrptitle{\myfigsetgrptitle{NGC~3344}}
\figsetplot{f2_19.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3344}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.20}
\figsetgrptitle{\myfigsetgrptitle{NGC~628}}
\figsetplot{f2_20.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~628}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.21}
\figsetgrptitle{\myfigsetgrptitle{NGC~4517}}
\figsetplot{f2_21.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4517}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.22}
\figsetgrptitle{\myfigsetgrptitle{NGC~3338}}
\figsetplot{f2_22.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3338}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.23}
\figsetgrptitle{\myfigsetgrptitle{NGC~5248}}
\figsetplot{f2_23.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~5248}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.24}
\figsetgrptitle{\myfigsetgrptitle{NGC~3198}}
\figsetplot{f2_24.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3198}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.25}
\figsetgrptitle{\myfigsetgrptitle{NGC~4631}}
\figsetplot{f2_25.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4631}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.26}
\figsetgrptitle{\myfigsetgrptitle{NGC~3486}}
\figsetplot{f2_26.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3486}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.27}
\figsetgrptitle{\myfigsetgrptitle{NGC~3556}}
\figsetplot{f2_27.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3556}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.28}
\figsetgrptitle{\myfigsetgrptitle{NGC~4559}}
\figsetplot{f2_28.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4559}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.29}
\figsetgrptitle{\myfigsetgrptitle{NGC~864}}
\figsetplot{f2_29.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~864}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.30}
\figsetgrptitle{\myfigsetgrptitle{NGC~660}}
\figsetplot{f2_30.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~660}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.31}
\figsetgrptitle{\myfigsetgrptitle{NGC~925}}
\figsetplot{f2_31.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~925}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.32}
\figsetgrptitle{\myfigsetgrptitle{NGC~4490}}
\figsetplot{f2_32.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~4490}}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.33}
\figsetgrptitle{\myfigsetgrptitle{NGC~3432}}
\figsetplot{f2_33.pdf}
\figsetgrpnote{\myfigsetgrpnote{NGC~3432}}
\figsetgrpend

\figsetend

